A Fixed-point Theorem for Horn Formula Equations

We consider constrained Horn clause solving from the more general point of view of solving formula equations. Constrained Horn clauses correspond to the subclass of Horn formula equations. We state and prove a fixed-point theorem for Horn formula equations which is based on expressing the fixed-point computation of a minimal model of a set of Horn clauses on the object level as a formula in first-order logic with a least fixed point operator. We describe several corollaries of this fixed-point theorem, in particular concerning the logical foundations of program verification, and sketch how to generalise it to incorporate abstract interpretations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{Hossein Hojjat and Bishoksan Kafle (Eds.): 8th Workshop on\\
Horn Clauses for Verification and Synthesis (HCVS 2021)
\\
EPTCS 344, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.344.5}{10.4204/EPTCS.344.5}}

